Built on Broken Assumptions (BOBA): Why Coding Agents Cannot Be Left Alone

Coding agents are autonomous developers. Given a request, they change the code and report back when done. As such, they can handle not only independent requests but whole chains of them, each request built on the last. Agents are known to report wrong work as done, yet benchmarks still test them one request at a time, on human-written code, checked once. We build BOBA-Bench, 280 chains of 20 consecutive requests drawn from 140 real open-source projects, and evaluate ten coding agents on both. All ten do far worse on chains. On average, they complete 95% of requests taken one at a time, but when requests are chained together, they complete 51%. Worse code is not the cause. Once checked, agent code is nearly as good a base for later requests as human code. The cause is the mistakes agents miss. Coding agents declare a request done once their own tests pass, even when those tests miss a mistake. The next request then builds on broken code and fails about twice as often. The mistake is rarely found later. Nor can agents catch such mistakes by reviewing code. Asked whether an implementation is correct, they are right 53% of the time, barely better than a coin flip. Coding agents are therefore heavily dependent on access to verification. A single external ``that's wrong'' after a failed request and one repair round lift chain completion from 51% to 59%, and a repaired mistake no longer hurts the requests that follow. In simpler terms, coding agents are only as reliable as the checks they can reach: without verification, every request that follows is built on broken assumptions.

==> boba_icons.tex <==
\makeatletter
\def\BobaIcon@agentcode{\includegraphics[height=0.95em]{figures/boba_icon_agentcode.pdf}}
\def\BobaIcon@autonomous{\includegraphics[height=0.95em]{figures/boba_icon_autonomous.pdf}}
\def\BobaIcon@continuation{\includegraphics[height=0.95em]{figures/boba_icon_continuation.pdf}}
\def\BobaIcon@humancode{\includegraphics[height=0.95em]{figures/boba_icon_humancode.pdf}}
\def\BobaIcon@review{\includegraphics[height=0.95em]{figures/boba_icon_review.pdf}}
\def\BobaIcon@verified{\includegraphics[height=0.95em]{figures/boba_icon_verified.pdf}}
\DeclareRobustCommand{\BobaMark}[1]{\raisebox{-0.12em}[0pt][0pt]{\@nameuse{BobaIcon@#1}}\nobreak\hspace{0.18em}}
\makeatother
\DeclareRobustCommand{\BobaTitleMark}{\raisebox{-0.15em}[0pt][0pt]{\includegraphics[height=1.15em]{figures/boba_icon_boba.pdf}}\nobreak\hspace{0.2em}}
\pdfstringdefDisableCommands{\def\BobaMark#1{}\def\BobaTitleMark{}}

